Assessing SSL/TLS Certificate Centralization: Implications for Digital Sovereignty

SSL/TLS is a fundamental technology in the network protocol stack that enables encrypted data transmission and authentication of web domains. However, the current model relies on a small number of Certificate Authorities (CAs) to provide and validate certificates, thus creating a highly centralized ecosystem. In this paper, we analyze the degree of centralization of certificate provisioning from CAs in two major political groups: Brazil, Russia, India, China, and South Africa (BRICS) and the European Union (EU). We have found that over 75% of certificates for both BRICS and EU domains originate from CAs based in the United States, indicating possible risks to their digital sovereignty due to the high level of external dependency. This indicates the need for nations within those groups to research alternatives to reduce the high level of dependency on foreign CAs and increase their digital autonomy.

==> methodology.tex <==
\section{Measurement Approach}
\label{sec:mesapp}

\newcommand*\rot{\multicolumn{1}{R{45}{1em}}}% no optional argument here, please!


The approach is based on collecting popular Internet domains from countries belonging to the EU and BRICS and fetching their certificate chain to inspect characteristics such as \1 the organization that issued the certificates (i.e., the Certificate Authority (CA)), \2 the certificate issuers countries of origin and \3 both start and expiration date for each certificate. Table~\ref{tab:sample-data} presents sample data collected from a domain obtained from the list of popular internet domains.

\begin{table}[h]
  \centering
  \caption{Certificate Information Example}
  \label{tab:sample-data}
  \begin{tabular}{r|c}
  \hline
    \textbf{Data Type} & \textbf{Example} \\ \hline
    \textit{Domain} & \texttt{www.wikipedia.org} \\ \hline
    \textit{Subject} & \texttt{CN=*.wikipedia.org} \\ \hline
    \textit{Issuer} & \makecell{\texttt{CN=}DigiCert TLS Hybrid ECC SHA384 2020 CA1 \\ \texttt{O=}DigiCert Inc \\ \texttt{C=US}} \\ \hline
    \textit{Serial} & 7f2f35c87a877af7aefe947993525bd \\ \hline
    \textit{Not Before} & 2021-04-14 00:00:00 \\ \hline
    \textit{Not After} & 2031-04-13 23:59:59 \\ \hline
\end{tabular}
  
\end{table}

The subject field identifies the entity that owns the certificate. It can contain information such as the Common Name (CN), representing the domain name of the entity; Organization (O), to identify the organization that holds the certificate; and Country (C), for the country of the entity. The \textit{Issuer} field represents the CA that issued the certificate, and contains the same fields: CN, for the name of the CA; O, for the CA organization; and C, for the country of origin of that CA. \textit{Serial} is a unique identifier for the emitted certificate within the responsible CA, and it ensures that they can be tracked and revoked individually. \textit{Not Before} and \textit{Not After} fields define, respectively, the earliest date and time when the certificate becomes valid, and the latest date and time that a certificate should be considered valid. After this period, a certificate can no longer be considered as trusted.

Figure~\ref{fig:sslchain-example} depicts a sample of the SSL/TLS certificate ecosystem using popular website domains.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{figs/background/sslchain.drawio.pdf}
    \caption{SSL/TLS Certificate Chain Example}
    \label{fig:sslchain-example}
\end{figure}

Each HTTPS domain should present an SSL/TLS certificate, which is the leaf certificate. It is issued to a website through an Intermediate CA and contains information about the server's public key and the owner of the server. An Intermediate CA acts as a middleware between the domain and the Root CA, by signing certificates using its private key and establishing a hierarchy from the Root CA to the server. Hence, the Root CA is the highest level in the certificate chain. It signs certificates for Intermediate CAs, thus completing the chain of trust from a domain up to the Root CA. Therefore, it is possible to traverse the certificate chain from the leaf, present in the domain, to its Root CA.

The defined approach presented in this section allows us to analyze the overall status of centralization of SSL/TLS certificate provision for domains in the political blocks of BRICS and EU, and to further investigate its possible impacts on the network sovereignty of the countries that compose them. Additionaly, it provides technical data to the geopolitical and economical discussion on digital sovereignty, thus facilitating further investigation on the topic. Figure~\ref{fig:approach} depicts the framework of the proposed methodology.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{figs/methodology/approach.drawio.pdf}
    \caption{Overview of the Approach}
    \label{fig:approach}
\end{figure}



The first step of Figure~\ref{fig:approach} consists of obtaining a list containing popular domains from countries within those political blocks. These types of lists are commonly used in research to perform measurements of the web and to evaluate prototypes~\cite{topplingLists, Le_Pochat_2019}. The second step encompasses obtaining the chain of certificates from each domain in the list of popular websites and storing this data. As shown in Figure~\ref{fig:sslchain-example}, by obtaining the leaf certificate present in a website, it is possible to traverse the certificate chain going through intermediate CAs until reaching the root CA. After processing the list of domains and storing their certificate chains, statistics can be retrieved from the data obtained. 

The implementation of the proposed framework and the results of the evaluation performed are publicly available in an anonymous way at~\cite{gitrepository}. In our solution, we relied on the Chrome User Experience Report (CrUX) dataset, which contains the top million most popular websites reported by Google Chrome~\cite{crux}. Although there are other lists such as Alexa Top Million and Tranco Top Million, the CrUX list seems to be the most accurate for assessing web popularity~\cite{topplingLists}. In order to retrieve the certificate chain from domains present in the domain list dataset, our solution creates a socket connection to each one of them through the SSL Python library, which provides a wrapper for the OpenSSL system-native library, and allows us to access SSL/TLS encryption and certificate facilities. Hence, it is possible to fetch the certificate chain of website domains and store them in a CSV file for further analysis. A mechanism of retry is implemented, in case that the socket connection fails to be established or any errors occurs during the certificate retrieval. If the errors persist, then the domain gets excluded from the final database.
